Synthesis with Asymptotic Resource Bounds

We present a method for synthesizing recursive functions that satisfy both a functional specification and an asymptotic resource bound. Prior methods for synthesis with a resource metric require the user to specify a concrete expression exactly describing resource usage, whereas our method uses big-O notation to specify the asymptotic resource usage. Our method can synthesize programs with complex resource bounds, such as a sort function that has complexity O(nlog(n)). Our synthesis procedure uses a type system that is able to assign an asymptotic complexity to terms, and can track recurrence relations of functions. These typing rules are justified by theorems used in analysis of algorithms, such as the Master Theorem and the Akra-Bazzi method. We implemented our method as an extension of prior type-based synthesis work. Our tool, SynPlexity, was able to synthesize complex divide-and-conquer programs that cannot be synthesized by prior solvers.

==> 3_background.tex <==
\section{Background}
\heping{In this section, we introduce the background }
\subsection{Recurrences Relations}


\begin{theorem}[Master Theorem \cite{bibid}]
	Let $m$ be an integer greater than or equal to 1 and $k$ be an integer greater than 1. Let $c$ be a positive real number and $d$ a nonnegative real number. Given a recurrence of the form
	\begin{equation*}
	T(n) = \begin{cases}
	mT(n/k)+U(n) &if\ n>1\\
	d & if\  n=1
	\end{cases}
	\end{equation*}
	then for $n$ a power of $k$
	\begin{enumerate}
		\item if $U(n)=O(n^{\log_{b}a-\epsilon})$ for some constant $\epsilon<0$, then $T(n)=\Theta(n^{\log_km})$,
		\item if $U(n)=\Theta(n^{\log_{b}a}\log^cn)$ with $c\ge0$, then $T(n)=\Theta(n^{\log_km}\log^{c+1} n)$,
		\item if $U(n)=\Omega(n^{\log_{b}a+\epsilon})$ with $\epsilon>0$ and $U(n)$ satisfies the regularity condition, then $T(n)=\Theta(U(n))$.
		Regularity condition: $mU(n/k)\le cU(n)$ for some constant $c<1$ and all sufficiently large $n$.
	\end{enumerate}
	\label{thm:master}
\end{theorem}
Besides Master Theorem, we can synthesis with other recurrence relation. The key idea is tracking the number of calls to subproblems, the size of each subproblem, and the cost of the merge function.


Let's first look at a variant of Master Theorem.
\begin{theorem}[Master Theorem \textnormal{(for subtract and conquer recurrences)}]
	Let $T(n)$ be a function defined on positive $n$, and having the property 
	\begin{equation*}
	T(n) \le \begin{cases}
	aT(n-b)+f(n) &if\ n>1\\
	c & if\  n\le 1
	\end{cases}
	\end{equation*}
	for some constants $c,a>0,b>0,d\ge0$, and function $f(n)$. If $f(n)$ is in $O(n^d)$, then
	\begin{equation*}
	T(n) \ is\ in\  \begin{cases}
	O(n^d) &if\ a<1\\
	O(n^{d+1}) & if\  a=1\\
	O(n^da^{n/b}) & if\ a>1
	\end{cases}
	\end{equation*}
\end{theorem}
For the Master Theorem for subtract and conquer recurrences, the sizes of subproblems will be $n-b$ instead of $n/b$.






Actually, the above two theorem are instances of a more general method reasoning recurrence formulas.
The Akra–Bazzi method applies to recurrence formulas of the form
$$T(x)=g(x) + \sum_{i=1}^k a_i T(b_i x + h_i(x))$$
The conditions for usage are:
\begin{itemize}
	\item sufficient base cases are provided
	\item $a_i$ and $b_i$ are constants for all $i$; $a_i > 0$ for all $i$; $0 < b_i < 1$ for all $i$
	\item $\left|g(x)\right| \in O(x^c)$, where ''c'' is a constant and ''O'' notates [[Big O notation]]
	\item $\left| h_i(x) \right| \in O\left(\frac{x}{(\log x)^2}\right)$ for all $i$
	
\end{itemize}



\begin{figure*}[h!]
	\includegraphics[width=\linewidth  ]{SynthesisWithRecursionRelation.pdf}	
	\caption{Architecture of synthesis with recurrences relations.}
\end{figure*}


\subsection{Asymptotic Resource Usage}
In this section, we will introduce the language we consider in this paper and the asymptotic cost of a program in that language.
\heping{What is resource usage? what is asymptotic usage bound?

Approximated 1 page}

==> 5_implementation.tex <==
\section{Implementation}
\heping{How do we extend existing solvers with \name. Approximated 1 page}

==> a1_semantics.tex <==
\section{Semantics}
\label{Se:aSemantics}

\mypar{Concrete semantics.} Here are all the evaluation judgments.
$${\inferrule*[right=\textsc{Sem-App }]
	{ \overline{v}~\text{are values}}
	{\concreteConfig{(\texttt{fix}~f.\lambda \overline{x}.t)\overline{v},C} \hookrightarrow \concreteConfig{[(\texttt{fix}~f.\lambda \overline{x}.t)/f][\overline{v}/\overline{x}]t,C}}
}$$ 

$${\inferrule*[right=\textsc{Sem-App-Arg }]
	{ \concreteConfig{t_1,0} \hookrightarrow \concreteConfig{t_2,C_\Delta}}
	{\concreteConfig{(\texttt{fix}~f.\lambda \overline{x}.t)t_1,C} \hookrightarrow \concreteConfig{(\texttt{fix}~f.\lambda \overline{x}.t)t_2,C+C_\Delta}}
}$$ 


$${\inferrule*[right=\textsc{Sem-Cond-True }]
	{ }
	{\concreteConfig{\texttt{if}~\texttt{true}~\texttt{then}~t_1~\texttt{else}~t_2,C} \hookrightarrow \concreteConfig{t_1,C}}
}$$ 

$${\inferrule*[right=\textsc{Sem-Cond-False }]
	{ }
	{\concreteConfig{\texttt{if}~\texttt{False}~\texttt{then}~t_1~\texttt{else}~t_2,C} \hookrightarrow \concreteConfig{t_2,C}}
}$$ 

$${\inferrule*[right=\textsc{Sem-Cond-Guard}]
	{ \concreteConfig{t_c,0} \hookrightarrow^* \concreteConfig{b,C_{\Delta}}\quad b~\text{is a Boolean value}}
	{\concreteConfig{\texttt{if}~t_c~\texttt{then}~t_1~\texttt{else}~t_2,C} \hookrightarrow \concreteConfig{\texttt{if}~b~\texttt{then}~t_1~\texttt{else}~t_2,C+C_\Delta}}
}$$ 

$${\inferrule*[right=\textsc{Sem-Match}]
	{ \overline{v}~\text{are values}}
	{\concreteConfig{\texttt{match}~\texttt{C}_j(\overline{v})~\texttt{with}~|_i\texttt{C}_i(\overline{x}_i) \mapsto  t_i,C} \hookrightarrow \concreteConfig{[\overline{v}/\overline{x}_i]t_i,C}}
}$$ 

$${\inferrule*[right=\textsc{Sem-Match-Scrutinee}]
	{ \concreteConfig{t_s,0} \hookrightarrow^* \concreteConfig{\texttt{C}_j(\overline{v}),C_{\Delta}}\quad \overline{v}~\text{are  values}}
	{\concreteConfig{\texttt{match}~t_s~\texttt{with}~|_i\texttt{C}_i(\overline{x}_i) \mapsto  t_i,C} \hookrightarrow \concreteConfig{\texttt{match}~\texttt{C}_j(\overline{v})~\texttt{with}~|_i\texttt{C}_i(\overline{x}_i) \mapsto  t_i,C+C_\Delta}}
}$$ 



\mypar{Polynomial-Bounded Refinement Type.}
The resource usage of a function call depends on the size of the problem it makes calls to. However, predicates used to refine functions could be imprecise, and thus we may have to reason about sizes of problems with imprecise refinements. For example, consider a function $\texttt{square::}\langle\texttt{Int}\to\{\texttt{Int}~|~\emph{v}\ge0\},\generatecolor{(O( \emph{v}))}\rangle$, where all we know about $\texttt{square}$ is that it returns a non-negative integer with linear resource usage  with respect to its input. In the nested application  term $\texttt{square}~(\texttt{square}~\texttt{x})$, we know the size of the problem of the inner application is $\texttt{x}$, but we do not know the size of the problem $\texttt{square~x}$ of the outer application (all we know about $\texttt{square~x}$ is that it is non-negative).
To reason about input sizes, we introduce a  class of refinement types with which we can infer upper bounds of the sizes of problems.


Let us first assume that all terms and variables  are integers or integer functions (we will discuss the case where terms and variables hold values other than integers later). For an integer refinement type $\tau=\{\texttt{Int}~|~\varphi\}$ refined by a predicate $\varphi(\emph{v},\overline{x})$ over $\emph{v}$ and a tuple of variables $\overline{x}$, we say that $\varphi$ is \emph{bounded} by a \emph{polynomial} term $p(\overline{x})$, written as $\varphi\bound p$ if 
$$\exists\overline{c}>\overline{0}\forall\overline{x}\forall\emph{v}.~\overline{x}\!>\!\overline{c}\wedge\varphi(\emph{v},\overline{x})\implies |\emph{v}|<p(\overline{x}).$$
That is, there exist some positive constants $\overline{c}$ such that, for any $\overline{x}$ (point-wise) greater than $\overline{c}$ and for any $\emph{v}$, if $\emph{v},\overline{x}$ satisfying $\varphi$, the absolute value $|\emph{v}|$ is always less than $p(\overline{x})$. 
\iffalse
Similarly, an  arrow type $\tau_\texttt{f}::x\!:\!\tau_1\!\to\!..\!\to\!x_n\!:\!\tau_n\to\tau$ is bounded by a polynomial $p$ if $\tau$ is bounded by $p$ with the refinements of arguments as context:
$$\exists\overline{c}.\forall\overline{x}.\forall\emph{v}.\overline{x}\!>\!\overline{c}\wedge\varphi(\emph{v},\overline{x})\wedge\bigwedge_{i=1}^n[x_i/v]\varphi_i\implies \emph{v}<p(\overline{x}), $$
where $\varphi_i$ is the refinement in $\tau_i$. 
\fi
\begin{example}
	The refinement type $\tau:=\{\texttt{Int}~|~\emph{v}\le 2x+y\vee\emph{v}\le x+2y\}$ is bounded by the expression $p_1:=2x+2y$ and the expression $p_2:=3x+3y$ but not $p_3:=2x+y+1$, i.e., $\tau\bound p_1$,~$\tau\bound p_2$, and $\tau\not\sqsubset p_3$.
\end{example}

For datatype $D$ other than $\texttt{Int}$, we assume that there is an \emph{intrinsic measure} with output type $\texttt{Int}$ for every $D$, denoted by $|\!\cdot\!|_D$ (we omit the subscript if it is clear from the context). Intrinsic measures are specified by users for user-defined datatypes. For example, the intrinsic measure of lists can be defined as a function that computes the length of lists, i.e., $|l|=\texttt{len}~l$ for any list $l$. The instinct measure of $\texttt{Int}$ term is the absolute-value function. The condition of $p$ bounding $\tau=\{D~|~\varphi(\emph{v},\overline{x})\}$ becomes
$$\exists\overline{c}>\overline{0}\forall\overline{x}\forall\emph{v}~\overline{|x|}\!>\!\overline{c}\wedge\varphi(\emph{v},\overline{x})\implies |\emph{v}|<p(\overline{|x|}). $$



\mypar{A loose cost model.}  
The semantics given previously give a standard notion of complexity. However, we find two challenges connecting these semantics to our synthesis algorithm. First, we allow users to supply auxiliary functions as signatures involving big-O notation as opposed to implementations. Second, our synthesis algorithm ensures complexity through the tracking of recursive calls, which are not present in the concrete semantics given above. To address these challenges we introduce an intermediate semantics that uses recurrence relations and big-O notation. We then show in \theoref{looseIsSound} that this intermediate semantics approximates complexity in the sense of \defrefs{complexity}{bigO}.

The signatures of auxiliary functions $f$ are of form $\langle\tau_1\to\{B~|~\varphi(\emph{v},\overline{y})\},\generatecolor{O(\psi(\emph{u}))}\rangle$.  Although we don't really have the implementation of $f$, we assume that there exists some implementation $\texttt{fix}~f.\lambda \overline{y}.t$ of $f$, such that
\begin{itemize}
	\item for any input $\overline{x}$, the output of $f$ on $\overline{x}$ satisfies the signature, i.e., $\concreteConfig{(\texttt{fix}~f.\lambda \overline{y}.t)\overline{x},0}\mapsto^*\concreteConfig{v_{\overline{x}},C_{\overline{x}}}$ implies $\varphi(v_{\overline{x}},\overline{x})$; and
	\item  for any input $\overline{x}$, the complexity  of $f$ is bounded by $\psi(\emph{u})$, i.e., $T_f(n)\in O(\psi(n))$.
\end{itemize}



Now we introduce our intermediate semantics. Formally, reductions are defined between configurations. Each configuration $\config{\hat{t},\checkcolor{\mathcal{R}}}$ is a pair of an extended term $\hat{t}$ and a recurrence parameter $\mathcal{R}$. Extended terms $\hat{t}::=t~|~\varphi$ are either terms $t$ or  formula expressions $\varphi$. Recurrence parameters $\mathcal{R}::=\phi~|~\bot~|~\mathcal{R}\!\parallel\!\mathcal{R}$ \john{I think you should be more explicit here. Don't recurrence parameters just consist of $\parallel$, $+$, ints, $T(x)$, and $\bot$. We can leave the $\le$ out till the end.} \heping{Recurrence parameters can also be polynomial over variables or any other size expressions.}are either size expressions $\phi$, or parameters combined by a \emph{parallel} operator $\parallel$, i.e., $\mathcal{R}$ is a collection of size expressions.    
The parallel operator $\parallel$ distributes over the plus operator, i.e., $(\mathcal{R}_1\parallel\mathcal{R}_2)+\mathcal{R}_3=\mathcal{R}_1+\mathcal{R}_2\parallel \mathcal{R}_1+\mathcal{R}_3$. Intuitively, a parameter $\mathcal{R}$ without parallelism denotes the recurrence relation of the function along one path. When the function contains more than one path, the overall parameter will be sub-parameters in parallel.




We use $\config{t,\checkcolor{\mathcal{R}}}\mapsto\config{\varphi,\checkcolor{\mathcal{R}'}}$ to denote a step of a reduction.  The goal is to reduce a term $t$ in a function $\texttt{f}$ to a predicate $\varphi$ such that $\varphi$ describes the behavior of $t$---$\varphi$ is a refinement of $t$. At the same time,  recurrence relations can be built  by incrementally appending expressions representing  resource usage to the recurrence parameter $\mathcal{R}$.
\john{In all of the premises of rules in the remainder of this section, $\mapsto^*$ can be replaced by $\mapsto$.}
\Omit{
\john{We had a comment that got removed about whether you need the $\mapsto^*$ or not in the concrete semantics. I originally said you didn't. However at the time I left that comment you hadn't added the sem-app-arg rule yet. Essentially with the rule as you have it, you do need the $\mapsto^*$ because now terms reduce in multiple steps. As you have it the concrete semantics are small step. But the loose semantics as you have them now are big step semantics. In the conclusion of each rule of the loose semantics every subterm gets reduced to a value (a formula) in one step. Furthermore, each subterm in each rule also gets reduced to a value. Thus there are no intermediate subterms that would ever be constructed. You can contrast the small step concrete semantics with the big step loose semantics with an example \texttt{if true then (add1 5) else 5}. In the concrete semantics we apply Sem-Cond-True and get \texttt{add1 5} which needs to be reduced further. However, in the loose semantics rule LooseSem-Cond \texttt{add1 5} would have already been reduced to a formula in the hypothesis of the inference rule. Thus when we apply the LooseSem-Cond rule we immediately get a result $v = 6$ in one step. The overall conclusion with this comment is that you do need the $*$ with the concrete semantics because they are small step, but you don't need it with the loose semantics because they are big step. But you can leave the $*$ in the loose semantics and it will still be fine. Just unnecessary.}}

Because we are building recurrence relations for a function $\texttt{f}$, the reduction always starts from a $\texttt{\textbf{fix}}$-term and an empty parameter $\bot$. The result configuration is the refinement $\varphi$ of the function body $t$  with the recurrence parameter $\checkcolor{ \mathcal{R}}$. We use the function $T:\texttt{Int}\to\texttt{Int}$ to denote the resource usage of the function $\texttt{f}$; hence, the recurrence parameter we build for $\texttt{f}$ will be the recurrence relation of resource usage $T$.
$${\inferrule*[right=\textsc{LooseSem-Fix }]
	{\config{t,0}\mapsto^* \config{\varphi,\mathcal{R}} }
	{\config{\texttt{\textbf{fix}~f}.\lambda x_1..\lambda x_n.t,~\bot}\mapsto \config{\varphi,~\checkcolor{ \mathcal{R}}}}
}$$ 

In our cost semantics, each auxiliary function $g$ has a resource annotation $\generatecolor{(O(\psi_g))}$ denoting the resource usage of $g$, a logical signature $\varphi_g$ denoting the behavior of $g$, and a size function $\texttt{size}_g$. Resource usage happens  when an auxiliary function is called.
$${\inferrule*[right=\textsc{LooseSem-App-Aux}]
	{
		g\!:\!\langle x_1\!:\!\tau_1\!\to\!..\!\to\!x_n\!:\!\tau_n\!\to\!\{B~|~\varphi_g\},\generatecolor{O(\psi_g)} \rangle\\  \forall i.\config{e_i,0}\mapsto^*\config{\varphi_i,\mathcal{R}_i}\qquad\varphi:= \varphi_g\wedge\bigwedge_{i=1}^n[x_i/\emph{v}]\varphi_i\quad
		\forall i.\varphi_i\bound v_i}
	{\config{g~e_1..~e_n,0}\mapsto \config{\varphi,\checkcolor{~[(\texttt{size}_g~v_1..~v_n)/\emph{v}]\psi_g+\sum_{i=1}^n\mathcal{R}_i}}}
}$$
That is, if each callee $e_i$ can be reduced to a predicate $\varphi_i$ bounded by $v_i$ with the recurrence parameter change $\mathcal{R}_i$, the non-recursive application term  $g~e_1..~e_n$ will be reduced to the predicate $\varphi$ with resource usage  $[\texttt{size}_g~v_1..~v_n/\emph{v}]\psi_g$ (the resource usage of $g$) and $\sum_{i=1}^n\mathcal{R}_i$ (resource usage used to evaluate $\{e_i\}_i$). We over-approximate the size of the problem $e_1..e_n$ using the upper bounds $v_i$ of callee's behavior predicates $\varphi_i$. The result predicate $\varphi$ is actually the behavior $\varphi_g$ of $g$ with each argument $x_i$ instantiated with the semantic predicates $[x_i/\emph{v}]\varphi_i$ of callee $e_i$.

The semantics of performing a recursive call is a bit different. The resource usage is instead $\checkcolor{T(\texttt{size}_\texttt{f}~v_1..~v_n)}$---the resource usage $T$ on a sub-problem with size  $\texttt{size}_\texttt{f}~v_1..~v_n$ where the $v_i$'s are over-approximations of the callee $e_i$'s.
$${\inferrule*[right=\textsc{LooseSem-App-Rec }]
	{ \forall i.\config{e_i,0}\mapsto^*\config{\varphi_i,\mathcal{R}_i} \qquad 
		\forall i.\varphi_i\bound v_i 	\\
		\texttt{f}\!:\!\langle x_1\!:\!\tau_1\!\to\!..\!\to\!x_n\!:\!\tau_n\!\to\!\{B~|~\varphi_\texttt{f}\},\generatecolor{O(\psi_\texttt{f})} \rangle\qquad\varphi:= \varphi_\texttt{f}\wedge\bigwedge_{i=1}^n[x_i/\emph{v}]\varphi_i}
	{\config{\texttt{f}~e_1..~e_n,0}\mapsto \config{\varphi,~\checkcolor{T(\texttt{size}_\texttt{f}~v_1..~v_n)+\sum_{i=1}^n\mathcal{R}_i}}}
}$$

The reduction of \texttt{if}-terms will result in $\texttt{ite}$ predicates. The resulting recurrence parameter $\checkcolor{\mathcal{R}_e+\mathcal{R}_1\parallel\mathcal{R}_e+\mathcal{R}_2}$ uses the parallel operator because there are two paths in an \texttt{ite} term.
$${\inferrule*[right=\textsc{LooseSem-Cond }]
	{\config{e,0}\mapsto^*\config{\varphi_e,\mathcal{R}_e}\quad\config{t_1,0}\mapsto^*\config{\varphi_1,\mathcal{R}_1}\quad\config{t_2,0}\mapsto^*\config{\varphi_2,\mathcal{R}_2}\\ \varphi:=\texttt{ite}~\varphi_e~\varphi_1~\varphi_2}
	{\config{\texttt{\textbf{if}}~e~\texttt{\textbf{then}}~t_1~\texttt{\textbf{else}}~t_2,0}\mapsto \config{\varphi,~\checkcolor{\mathcal{R}_e+\mathcal{R}_1\parallel\mathcal{R}_e+\mathcal{R}_2}}}
}$$

With the above rules, we can then say the complexity of a function to be any expression that satisfy the recurrence parameter of the function.



\begin{theorem}[Complexity bounds]\label{The:looseIsSound}
	Given a function term $\texttt{\textbf{fix}~f}.\lambda \overline{x}.t$, if 
	\begin{itemize}
		\item the function body $t$ can be reduced to $\config{\cdot,\mathcal{R}}$, where $\mathcal{R}$ is of form $\mathcal{R}_1\parallel..\parallel\mathcal{R}_m$, and none of the $\mathcal{R}_i$'s contain an occurrence of the parallel operator; and
		\item there exists a function $\psi$ that satisfies
\[
  \forall i.T(\texttt{size}_\texttt{f}(\overline{x}))\le\mathcal{R}_i\implies T(\texttt{size}_{\texttt{f}}(\overline{x}))\in O(\psi(\texttt{size}_{f}(\overline{x}))),
\]
	\end{itemize} then the complexity $T_f$ of $\texttt{f}$ is bounded by the function $\psi$, i.e., $T_f\in O(\psi)$.
\end{theorem}
\john{Are you going to prove this?}

\begin{example}
	For the program shown in 
	\eqref{prod_log}, there are three paths. At the beginning, $\texttt{\textbf{fix}~prod}.\lambda x.\lambda y.t $ is reduced to $\config{\varphi,\checkcolor{T(\texttt{size}_{\texttt{\textbf{prod}}}~x~y)\le 0+\mathcal{R}}}$ where $\mathcal{R}$ is the reduction result of the function body, and $\texttt{size}_{\texttt{\textbf{prod}}}~x~y=x$ since the size function for \texttt{prod} is $\lambda z.\lambda w.z$
	
	The first \texttt{ite} term $\texttt{\textbf{if}}~x==0~\texttt{\textbf{then}}~t_1~\texttt{\textbf{else}}~t_2$ is reduced to $\config{\texttt{ite}(x==0,~\varphi_1,~\varphi_2),\checkcolor{\mathcal{R}_e+\mathcal{R}_1\parallel\mathcal{R}_e+\mathcal{R}_2}}$ where the condition contain one equivalence operator ($\mathcal{R}_e=1$), the \texttt{then} branch has 0 resource usage (it is a variable term) ($\mathcal{R}_1=0$), and the \texttt{else} branch has resource usage $\mathcal{R_2}$, which we learn from the reduction of $t_2$.
	
	The application term $\texttt{div2~}x$ is reduced to $\config{v=\frac{z}{2}\wedge z=x,~1}$ since the resource  usage of $\texttt{div2}$ is $O(1)$.
	
	The recursive-application term \texttt{prod~(div2~x)~y} is reduced to $\config{v=z*w\wedge z=\frac{x}{2}\wedge w= y,~\mathcal{R}_0+T(\frac{x}{2})+1}$
	
	Overall the recurrence relation can be built as
	$T(x)\le 1\parallel T(x)\le 4 +T(\frac{x}{2})\parallel T(x)\le 5+T(\frac{x}{2})$. Thus the complexity of $\texttt{prod}$ is bounded by $\log x$ since $T(x)\le1\implies T(x)\in O(\log x)$, and, $T(x)\le 5+T(\frac{x}{2})\implies T(x)\in O(\log x)$ according to the Master Theorem.
	
	
\end{example}


\mypar{Soundness theorem.}


The proof of the soundness theorem uses  the following crucial lemma connecting the recurrence annotations with the actual recurrence relations of functions.
\begin{lemma}
	\label{Lem:rec}
	Given a function $\texttt{fix }f.\lambda x_1..\lambda x_n.t$, if\ $\Gamma\vdash t\irefine \langle\tau;([c_1,\phi_1],..[c_m,\phi_m],O(\psi))\rangle$, then the complexity~$T$ of $f$ satisfies $T(v)\le c_1T(\phi_1)+..+C_mT(\phi_m)+O(\psi)$
\end{lemma}
\begin{proof}
The proof of the lemma consists two parts: 1) the recursive calls are tracked correctly, and 2) the bound on the function body is tracked correctly. We assume that the function $\texttt{fix }f.\lambda x_1..\lambda x_n.t$ can be reduced to the recurrence parameter $\mathcal{R}_1\parallel..\parallel\mathcal{R}_m$. In the branching rules \textsc{T-Match} and \textsc{T-If}, all branches share the same annotation $\alpha_2$. That is, the annotation $\alpha_2$ is the \emph{upper bound} of the recurrence parameters of all branches. 
	
	
For recursive calls, the implication predicate in the rule \textsc{E-RecApp} is stronger than polynomial bounds. In detail, if some polynomial $p$ bounds $\varphi_i$, then $\forall \overline{x}\forall y. [y/\emph{v}]\varphi_i(\overline{x})\implies y<p(\overline{x})$. Also, the subtyping rule \textsc{<:-Anno} ensures that sizes of subproblems can only be overapproximation. 
	
For auxiliary function calls, the implication predicate in the rule
\textsc{E-App} is stronger than polynomial bounds for the same reason
as above.
Also, big-O notation is closed under polynomial and substitutions.
\john{Not true that big-O notation is closed under substitutions.  It may be for some restricted set of substitutions that we rely on.}
\end{proof}

\begin{theorem}[Soundness of type checking]
	Given a function $\texttt{fix }f.\lambda x_1 \ldots \lambda x_n.t$ and an environment $\Gamma$, if $\Gamma\vdash \texttt{fix }f.\lambda x_1 \ldots \lambda x_n.t:: \langle\tau,\generatecolor{O(\psi)} \rangle$, then the complexity of $f$ is bounded by $\psi$.
\end{theorem}
\begin{proof}This theorem can be proved by combining \lemref{rec} and theorems used in the \tablename{pattern}.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main_cav.tex"
%%% End: 


==> a1_syntax.tex <==
\section{Syntax and Types}
\label{Se:aSyntax}

\begin{figure}[tb]
	\begin{mathpar}
		\boxed{\Gamma\vdash \tau<:\tau'}\hspace{5mm}
		{\inferrule*[right=\textsc{<:-Fun}]
			{\Gamma\vdash \tau_y<:\tau_x\qquad \Gamma;y:\tau_y\vdash[y/x]\tau<:\tau'}
			{ \Gamma\vdash x:\tau_x\to\tau~<:~y:\tau_y\to\tau'}
		}\\
		{\inferrule*[right=\textsc{<:-Sc}]
			{\Gamma\vdash B<:B'\qquad \Gamma\models\varphi\implies\varphi'}
			{ \Gamma\vdash \{B~|~\varphi\}<:\{B'~|~\varphi'\}}
		}\hspace{5mm}
		{\inferrule*[right=\textsc{<:-Refl}]
			{\ }
			{ \Gamma\vdash B~<:~B}
		}\\
		%		{\inferrule*[right=\textsc{<:-Anno}]
		%			{\Gamma\vdash \tau<:\tau'\qquad \Gamma\models [x/\emph{v}]\phi\wedge[x'/\emph{v}]\phi'\Rightarrow \%emph{x}'>\emph{x}\qquad \Gamma\models \psi\in O(\psi')}
		%			{ \Gamma\vdash \langle\tau,\generatecolor{([1,\phi];O(\psi))}\rangle<:\langle\tau',\generatecolor{([1,\phi'];O(\psi'))}}
		%		}
		\\
		{\inferrule*[right=\textsc{<:-Rec}]
			{ c'>c\quad \Gamma\models [x/\emph{v}]\phi\wedge[x'/\emph{v}]\phi'\Rightarrow \emph{x}'>\emph{x}}
			{ \Gamma\vdash \generatecolor{[c,\phi]}<:\generatecolor{[c',\phi']}}
		}\qquad
		{\inferrule*[right=\textsc{<:-Bound}]
			{ \Gamma\models \psi\in O(\psi')}
			{ \Gamma\vdash \generatecolor{O(\psi)}<:\generatecolor{O(\psi')}}
		}\\
		{\inferrule[\textsc{<:-Rec-Split}]
			{  \Gamma\models \phi_1=\phi_2}
			{  \Gamma\vdash \langle\tau',\generatecolor{([c_1+c_2,\phi_1],[c_3,\phi_3]\ldots[c_n,\phi_n];O(\psi))}\rangle<:\langle\tau,\generatecolor{([c_1,\phi_1],[c_2,\phi_2],\ldots[c_n,\phi_n];O(\psi))}\rangle}
		}\\
		{\inferrule[\textsc{<:-Rec-Combine}]
			{  \Gamma\models \phi_1=\phi_2}
			{  \Gamma\vdash \langle\tau,\generatecolor{([c_1,\phi_1],[c_2,\phi_2],\ldots[c_n,\phi_n];O(\psi))}\rangle<:\langle\tau',\generatecolor{([c_1+c_2,\phi_1],[c_3,\phi_3]\ldots[c_n,\phi_n];O(\psi))}\rangle}
		}\\{\inferrule*[right=\textsc{<:-Anno-Rec}]
			{\Gamma\vdash \tau<:\tau'\qquad \forall i .\Gamma\vdash \generatecolor{[c_i,\phi_i]}<:\generatecolor{[c'_i,\phi'_i]}\qquad \Gamma\vdash \generatecolor{O(\psi)}<:\generatecolor{O(\psi')}}
			{ \Gamma\vdash \langle\tau,\generatecolor{([c_1,\phi_1],\ldots[c_n,\phi_n];O(\psi))}\rangle<:\langle\tau',\generatecolor{([c_1',\phi_1']\ldots[c'_n,\phi'_n];O(\psi'))}\rangle}
		}\\ \heping{\text{maybe moved some of them above to the appendix}}
	\end{mathpar}
	\caption{Subtyping rules.}
	\label{Fi:subtype}
\end{figure}

\tom{There is some nearly duplicated text in the first two paragraphs.}
\mypar{Subtyping.} Subtyping judgments are shown in \figref{subtype}, and are standard. The most notable rule is \textsc{<:-Anno}, which states that bounds $\generatecolor{\psi'}$ and the sub-problems' size $\generatecolor{\phi'}$ in the annotations in subtypes should be less than in the supertype.

\begin{changebar}
	Subtying judgments are shown in \figref{subtype}, and are standard. The most notable rules are \textsc{<:-Rec} and \textsc{<:-Bound}, which states that bounds $\generatecolor{\psi}$ and the sub-problems' size $\generatecolor{\phi}$ in the annotations in subtypes should be less than in the supertype.
	\[	{\inferrule*[right=\textsc{<:-Rec}]
		{ c'>c\quad \Gamma\models [x/\emph{v}]\phi\wedge[x'/\emph{v}]\phi'\Rightarrow \emph{x}'>\emph{x}}
		{ \Gamma\vdash \generatecolor{[c,\phi]}<:\generatecolor{[c',\phi']}}
	}\\
	{\inferrule*[right=\textsc{<:-Bound}]
		{ \Gamma\models \psi\in O(\psi')}
		{ \Gamma\vdash \generatecolor{O(\psi)}<:\generatecolor{O(\psi')}}
	}\]
\tom{Are the occurrences of $\floor{\cdot}$ supposed to be $\ceil{\cdot}$?}
	For example, if one branch of some branching term has type $\langle\tau,(\generatecolor{[1,\floor{\frac{\emph{u}}{3}}],O(\psi)})\rangle$, it can be over-approximated by a super type $\langle\tau,(\generatecolor{[1,\floor{\frac{\emph{u}}{2}}],O(\psi)})\rangle$. The idea is that the resource usage of an application calling to a problem of size $\generatecolor{\floor{\frac{\emph{u}}{2}}}$, will be larger than the application calling to a smaller problem of size $\generatecolor{\floor{\frac{\emph{u}}{3}}}$, with the assumption that all resource usages are monotonic.
\end{changebar}


==> discard-introduction.tex <==
However, very little has been done on synthesizing programs with good
performance.
In this paper, we consider the problem of program synthesis under
a resource constraint---in particular, a constraint on asymptotic execution-time efficiency.
\john{I would remove the previous two sentences. We say many techniques, but only give one. Also I don't see how that work is relevant here. I would bring the next paragraph in an say something like. Recently \cite{knoth2019resource} examined synthesis with resource bounds using ...}

The problem of \emph{verifying} programs' asymptotic resource usage has been a longstanding theme in the verification community \john{You could put a million citations here if you wanted}. We consider proof-based analysis techniques that derive symbolic recurrence relations for a program's resource usage, and then connect the recurrence relations with asymptotic resource bounds using classical theorems such as the Master Theorem \cite{Book:CLR01}, the Akra-Bazzi method \cite{eberl2017proving}, or C-finite sequence analysis \cite{TACAS:Kovacs2008,PACMPL:KCBR18}. In this paper, we push the idea of proof-based resource analysis into program synthesis. 

\emph{Challenges.} 
One of the reasons that AARA and the use of exact bounds is a good fit for being adapted to type-directed synthesis techniques (as done in~\cite{}) is that we one share the exact resource bounds to sub-terms of the synthesized programs and reject sub-terms exceeding the bounds at an early stage. For example, you one share the bound $2n$ to two sub-goals to make each of them has bound $n$, or one of them has bound $2n$ and the other has bound $0$. But we cannot share asymptotic bounds such as $O(\log n)$ with the same idea. \john{I don't know what this paragraph is trying to say. Should the next paragraph go before this one?}

\john{That is this paragraph starts with ``We combine these prior resource analysis techniques with a type-directed synthesis algorithm to synthesize terms that meet a given asymptotic resource bound... This approach has some challenges...''}
\loris{I agree, we should say what we do and maybe later say a sentence about why it can be done vs AARA cannot. Most of this discussion should go to related}
We present a type-directed algorithm for synthesizing terms that meet a given asymptotic resource bound. Our algorithm proceeds in two steps. First, it guesses recurrence relations consistent with the given resource bound by using a pattern-matching-based recurrence relation inference rule. Then, it build terms satisfying the the guessed recurrence relations. Each step has a number of challenges.

\emph{From asymptotic bounds to recurrence relations.}
\loris{this is a bit too concrete and detailed for an intro. I would avoid bringing up heuristics so soon.}
 For any given asymptotic-resource bound there are many inference rules in our synthesizer that can be applied. For example, seeing a pattern $O(\log n)$, our Master-Theorem-based inference rules will tell that a recurrence relation of form $T(n)=T(\frac{n}{a})+O(1)$ implies $T(n)\in O(\log n)$ for any integer $a\ge 2$. We address this challenge by heuristically guessing $a$ starting from 2 to instantiate the recurrence relation the synthesized term should satisfy, for example, $T(n)=T(\frac{n}{2})+O(1)$, $T(n)=T(\frac{n}{3})+O(1)$, and so on.

\emph{Enumerating terms that satisfy a recurrence relation and functional specification.} Once a recurrence pattern has been selected, we want to have our synthesizer only generate terms that satisfy the chosen recurrence pattern. To address this challenge we augment a type system for functional programs with additional resource annotations. These additional annotations  denote the number of recursive calls we can make in the synthesized terms, the size of subproblems of recursive calls, and the resource bound of the top-level function. For example, a term with annotated type $\langle\tau,([1,\frac{n}{2}];O(1))\rangle$ has type functional type $\tau$, and satisfies the relation $T(n)\le T(\frac{n}{2})+O(1)$ since it contains \emph{one} recursive call to sub-problem with size $\frac{n}{2}$, and the top-level resource usage is bounded by $O(1)$. These additional annotations do not ensure the resulting term will be functionally correct, so we combine our system with other type-directed synthesis technique such as \synquid \cite{knoth2019resource} and \myth \cite{osera2015type} to synthesize terms that are both correct and satisfying the resource bound.

\emph{Synthesizing appropriate subproblems.} Another challenge is how to synthesize concrete recursive applications. For example, consider synthesizing an $O(n\log(n))$ sorting function $\texttt{msort}$, where $n$ is equal to the length of the input list, $|\texttt{l}|$. We could correctly guess a recurrence pattern of $T(n)=2T(\frac{n}{2})+O(n)$. This means our resulting term would have two recursive calls, each on an input of size $\frac{|\texttt{l}|}{2}$. However, it is still unclear how to construct the concrete recursive applications. That is, we will have two terms of the form $\texttt{msort}\ \ \texttt{??}$ where the ``size'' of the term that fills the hole must be $\frac{|\texttt{l}|}{2}$, but we don't directly have access to such terms. 
\loris{this paragraph is confusing and I'm not sure we have a good story here.
We really need refinement types to make sure our solution divides the input by 2. 
}
We address this challenge by using modularity synthesis \john{???} where we synthesize the terms of recursive calls independently using the size restrictions as specifications. In the example of merge sort, we know that we want to make two recursive calls to subproblems of size $\frac{|\texttt{l}|}{2}$. So we construct another synthesis problem to synthesize an auxiliary function $\texttt{split}$ with the specification that the size of the output should be half of the size of the input. Then the solution implementation of \texttt{split} will be an auxiliary function that converts the original problem to sub-problems with wanted size.



==> plot_searchSpace.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-8mm}
\centering
\begin{tikzpicture}[scale=0.6, every node/.style={transform shape}]
\begin{axis}[%
legend style={cells={align=left}},
%xmode=log,
%ymode=log,
label style={font=\Large},
ylabel= \tool,
xlabel= \synquid,
%xtick =data,
%xtick={1000,10000,100000,300000},
%xticklabels={$10^3$,$10^4$,$10^5$,$TO$},
scatter/classes={%
a={mark=*,draw=black,
mark options={solid},
mark size = 3pt,
style={solid, fill=white}}, b={mark=triangle*,draw=black,
mark options={solid},
style={solid, fill=white}, mark size = 4pt},
c={mark=x,draw=black,
mark options={solid}, mark size = 4pt,
style={solid, fill=white}}},
xmin = 0,
xmax = 20000,
ymin = 0,
ymax = 20000]
\addplot[scatter,only marks,%
scatter src=explicit symbolic]%
table[meta=label] {
x y label
9	7 a
186	186 a
145	145 a
86	86 a
170	162 a
111	111 a
42	42 a
120	120 a
73	72 a
851	843 a
204	204 a
113	110 a
137	137 a
57	57 a
584	579 a
2202	2029 a
78	75 a
625	625 a
449	444 a
13	11 a
128	128 a
1198	1198 a
636	624 a
950	932 a
614	614 a
1183	1062 a
2080	1929 a
3818	3630 a
6572	6560 a
16337	16337 a
};
\draw [solid, color=red] (0,0) -- (100,100);
%\addlegendentry{Polynomials}
%\addlegendentry{Repair}
%\addlegendentry{Invariant}
\end{axis}
\end{tikzpicture}
\caption{Number of E-terms enumerated during synthesis.  \label{Fi:searchSpace}}
\vspace{-6mm}
\end{wrapfigure}
